QCCDCert: Formally Verified Compilation for QCCD Co-Design

Quantum charge-coupled device (QCCD) architectures enable scalable trapped-ion quantum computing by dynamically shuttling ions between specialized processing and storage zones. A QCCD can be built with many trap sizes and layouts. Comparing them requires compiling every program under each design's transport, capacity and control constraints, and trusting the target code of each compilation. We present a co-design framework built on one Lean-verified compiler. The hardware description and its operating rules are compiler inputs, so a single theorem covers every candidate design: the target code of every compilation preserves its program's behavior and obeys the hardware rules. Across 75 benchmark programs of 11 to 130 qubits, the best design found takes 66% less modeled execution time on average than the worst design of equal capacity. An AI agent that proposes devices based on our compiler's checked results beats the fastest of these designs on 71 of 75 programs. Our verified compiler provably avoids the 11 defects that we report in three previous compilers. It scales to hundreds of qubits, compiling 512-qubit programs for a 38-trap device in 1 to 29 minutes.

==> qccd-hardware.tex <==
% Editable LaTeX port of the QCCD interactive studio's hardware grammar.
% Geometry: qccd/viz/layout.py and render.py::buildStatic / slotOffsets.
% Palette: qccd/viz/theme.py. See assets/hardware/README.md for provenance.
% No image files or converted SVG paths are used by these drawings.
\RequirePackage{tikz}
% Shared two-zone snapshots for the complete physical compiler example.
\newcommand{\QCCDTwoZoneSnapshot}[1]{%
  \begin{tikzpicture}[x=\QCCDUnit,y=-\QCCDUnit,transform shape]
    \QCCDGeometry{80}{20}
    % Keep identifiers at 8pt in the worked figure's 112pt snapshots.
    \def\qccd@font{13.6}\def\qccd@texthalo{1.1}
    \QCCDDeclareSite{S}{25}{25}{0}{qhwTrap}{1}{qhwTrap}
    \QCCDDeclareSite{G}{145}{25}{0}{qhwTrap}{2}{qhwTrap}
    \QCCDRail{S}{G}
    \QCCDDrawSite{S}\QCCDDrawSite{G}
    \QCCDSiteLabel{S}\QCCDSiteLabel{G}
    \ifnum#1=0
      \QCCDIon{q0}{S}{0}\QCCDIon{q1}{G}{1}
    \else
      \QCCDIon{q0}{G}{0}\QCCDIon{q1}{G}{1}
    \fi
    \ifnum#1=2
      \draw[qhwBeam,line width=2\QCCDUnit] (145,-12)--(145,13);
      \draw[qhwBeam,line width=1\QCCDUnit] (132,10)--(158,10);
    \fi
    \pgfresetboundingbox
    \path[use as bounding box] (-10,-17) rectangle (180,73);
  \end{tikzpicture}}
% Load T1 for hardware IDs without changing the paper's default OT1 encoding.
\RequirePackage[T1,OT1]{fontenc}
\RequirePackage[outline]{contour}
\usetikzlibrary{calc}
\newdimen\QCCDUnit
\QCCDUnit=.75bp % one CSS pixel; every geometry parameter below is in this unit
\definecolor{qhwInk}{HTML}{182230}
\definecolor{qhwRail}{HTML}{F2B8B5}
\definecolor{qhwCompute}{HTML}{9CCE9C}
\definecolor{qhwData}{HTML}{475467}
\definecolor{qhwTrap}{HTML}{0F766E}
\definecolor{qhwCorner}{HTML}{F6C34A}
\definecolor{qhwGold}{HTML}{E8B84B}
\definecolor{qhwGrid}{HTML}{8A94A6}
\definecolor{qhwElectrode}{HTML}{C3CBD8}
\definecolor{qhwLoop}{HTML}{4338CA}
\definecolor{qhwBeam}{HTML}{C2308A}
\makeatletter

% Public low-level API: declare a site, connect sites, and place an ion in a slot.
% IDs are both editable names and TikZ coordinates (T0_0h, C0, A0, ...).
% Site arguments: ID, x, y, axis angle, zone colour, capacity, outline colour.
\newcommand{\QCCDDeclareSite}[7]{%
  \coordinate (#1) at (#2,#3);
  \expandafter\def\csname qccd@x@#1\endcsname{#2}%
  \expandafter\def\csname qccd@y@#1\endcsname{#3}%
  \expandafter\def\csname qccd@axis@#1\endcsname{#4}%
  \expandafter\def\csname qccd@zone@#1\endcsname{#5}%
  \expandafter\def\csname qccd@cap@#1\endcsname{#6}%
  \expandafter\def\csname qccd@outline@#1\endcsname{#7}%
  \expandafter\edef\csname qccd@span@#1\endcsname{\qccd@sitespan}%
}
\newcommand{\QCCDDeclareJunction}[4]{%
  \coordinate (#1) at (#2,#3);
  \expandafter\def\csname qccd@x@#1\endcsname{#2}%
  \expandafter\def\csname qccd@y@#1\endcsname{#3}%
  \expandafter\def\csname qccd@outline@#1\endcsname{#4}%
  \expandafter\edef\csname qccd@span@#1\endcsname{\qccd@junctionradius}%
}
\newcommand{\QCCDLabel}[5][center]{%
  \begingroup
  \contourlength{\qccd@texthalo\QCCDUnit}%
  \node[anchor=#1,inner sep=0pt,outer sep=0pt,text=#4,
    font=\fontencoding{T1}\fontfamily{phv}\fontseries{b}\selectfont
      \fontsize{\qccd@font\QCCDUnit}{\qccd@font\QCCDUnit}\selectfont]
    at (#2,#3) {\contour{white}{\detokenize{#5}}};
  \endgroup
}
% Native dimensions: g is the shortest distance between two hardware nodes;
% electrode pitch is the technology's 58 um converted to the scene scale.
\newcommand{\QCCDGeometry}[2]{%
  \def\qccd@g{#1}\def\qccd@pitch{#2}%
  \pgfmathsetmacro\qccd@font{min(12,max(2.5,.18*#1))}%
  \pgfmathsetmacro\qccd@texthalo{.14*\qccd@font}%
  \pgfmathsetmacro\qccd@sitespan{1.5*#2}%
  \pgfmathsetmacro\qccd@junctionradius{.30*#1}%
  \pgfmathsetmacro\qccd@thickness{.083*2.4*#1}%
  % Round only the fractional part: multiplying a large spacing by 1000
  % otherwise exceeds PGF's fixed-point dimension range.
  \pgfmathsetmacro\qccd@thickness{int(\qccd@thickness)+round((\qccd@thickness-int(\qccd@thickness))*1000)/1000}%
  \pgfmathsetmacro\qccd@nodewidth{max(1,.05*#1)}%
  \pgfmathsetmacro\qccd@railwidth{max(1.2,.083*#1)}%
  \pgfmathsetmacro\qccd@padwidth{50/58*#2}%
  \pgfmathsetmacro\qccd@padoffset{.30*#1}%
  \pgfmathsetmacro\qccd@padthickness{.20*#1}%
}
% As on the website, a trap stops growing at six slots. \QCCDLongTraps keeps
% the slot pitch up to twelve slots, for drawings that show every ion place.
\def\qccd@slotcap{6}\def\qccd@lencap{.88}
\newcommand{\QCCDLongTraps}{\def\qccd@slotcap{12}\def\qccd@lencap{2.1}}
% An electrode pair is two rectangular pads, never rounded pills.
% Small thumbnails may switch the electrode pads off with \qccdpadsfalse.
\newif\ifqccdpads \qccdpadstrue
\newif\ifqccdionlabels \qccdionlabelstrue
\newcommand{\QCCDElectrodePair}[3]{%
  \ifqccdpads\begin{scope}[shift={(#1,#2)},rotate={-#3}]
    \foreach \side in {-1,1}{
      \path[fill=qhwElectrode,fill opacity=.42]
        ({-.5*\qccd@padwidth},{\side*\qccd@padoffset-.5*\qccd@padthickness})
        rectangle
        ({.5*\qccd@padwidth},{\side*\qccd@padoffset+.5*\qccd@padthickness});
    }
  \end{scope}\fi
}
% Each rail is a readable pair of endpoint IDs. Its electrode tiling follows
% the website exactly: site stacks reserve their span; rail pairs fill the rest.
\newcommand{\QCCDRail}[3][qhwRail]{%
  \edef\qccd@ax{\csname qccd@x@#2\endcsname}%
  \edef\qccd@ay{\csname qccd@y@#2\endcsname}%
  \edef\qccd@bx{\csname qccd@x@#3\endcsname}%
  \edef\qccd@by{\csname qccd@y@#3\endcsname}%
  \pgfmathsetmacro\qccd@distance{veclen(\qccd@bx-\qccd@ax,\qccd@by-\qccd@ay)}%
  \pgfmathsetmacro\qccd@angle{atan2(\qccd@by-\qccd@ay,\qccd@bx-\qccd@ax)}%
  \pgfmathsetmacro\qccd@run{\qccd@distance-\csname qccd@span@#2\endcsname-\csname qccd@span@#3\endcsname}%
  \pgfmathtruncatemacro\qccd@count{max(0,min(12,floor(\qccd@run/\qccd@pitch)))}%
  \def\qccd@colour{#1}\def\qccd@compute{qhwCompute}%
  \ifx\qccd@colour\qccd@compute
    \pgfmathsetmacro\qccd@width{max(1,.065*\qccd@g)}\def\qccd@opacity{.9}%
  \else\let\qccd@width\qccd@railwidth\def\qccd@opacity{1}\fi
  \ifnum\qccd@count=0
    \pgfmathsetmacro\qccd@gap{\qccd@pitch-\qccd@padwidth}%
    \draw[#1,opacity=\qccd@opacity,line width=\qccd@width\QCCDUnit,
      dash pattern=on \qccd@padwidth\QCCDUnit off \qccd@gap\QCCDUnit]
      (#2)--(#3);
  \else
    \draw[#1,opacity=\qccd@opacity,line width=\qccd@width\QCCDUnit,line cap=butt](#2)--(#3);
    \pgfmathsetmacro\qccd@start{\csname qccd@span@#2\endcsname+(\qccd@run-\qccd@count*\qccd@pitch)/2}%
    \foreach \i in {1,...,\qccd@count}{
      \pgfmathsetmacro\qccd@along{\qccd@start+(\i-.5)*\qccd@pitch}%
      \pgfmathsetmacro\qccd@px{\qccd@ax+cos(\qccd@angle)*\qccd@along}%
      \pgfmathsetmacro\qccd@py{\qccd@ay+sin(\qccd@angle)*\qccd@along}%
      \QCCDElectrodePair{\qccd@px}{\qccd@py}{\qccd@angle}
    }
  \fi
}
\newcommand{\QCCDDrawSite}[1]{%
  \edef\qccd@x{\csname qccd@x@#1\endcsname}%
  \edef\qccd@y{\csname qccd@y@#1\endcsname}%
  \edef\qccd@angle{\csname qccd@axis@#1\endcsname}%
  \edef\qccd@capacity{\csname qccd@cap@#1\endcsname}%
  \edef\qccd@zone{\csname qccd@zone@#1\endcsname}%
  \edef\qccd@outline{\csname qccd@outline@#1\endcsname}%
  \pgfmathsetmacro\qccd@length{min(\qccd@lencap*\qccd@g,(.30+.15*min(\qccd@slotcap,\qccd@capacity))*\qccd@g)}%
  \pgfmathsetmacro\qccd@radius{min(.085*\qccd@g,.36*\qccd@length/\qccd@capacity)}%
  \pgfmathsetmacro\qccd@ringwidth{min(max(.7,.8*\qccd@nodewidth),.8*\qccd@radius)}%
  \ifx\qccd@zone\qccd@outline
    \let\qccd@width\qccd@nodewidth\def\qccd@opacity{.55}%
  \else
    \pgfmathsetmacro\qccd@width{1.7*\qccd@nodewidth}\def\qccd@opacity{.95}%
  \fi
  \foreach \offset in {-1,0,1}{
    \pgfmathsetmacro\qccd@px{\qccd@x+cos(\qccd@angle)*\offset*\qccd@pitch}%
    \pgfmathsetmacro\qccd@py{\qccd@y+sin(\qccd@angle)*\offset*\qccd@pitch}%
    \QCCDElectrodePair{\qccd@px}{\qccd@py}{\qccd@angle}
  }
  \begin{scope}[shift={(#1)},rotate={-\qccd@angle}]
    \pgfmathsetmacro\qccd@corner{.5*\qccd@thickness}%
    \path[rounded corners=\qccd@corner\QCCDUnit,fill=\qccd@zone,fill opacity=.16,
      draw=\qccd@outline,draw opacity=\qccd@opacity,line width=\qccd@width\QCCDUnit]
      ({-.5*\qccd@length},{-.5*\qccd@thickness})
      rectangle ({.5*\qccd@length},{.5*\qccd@thickness});
    \pgfmathtruncatemacro\qccd@last{\qccd@capacity-1}%
    \foreach \i in {0,...,\qccd@last}{
      \coordinate (#1-slot-\i) at ({((\i+.5)/\qccd@capacity-.5)*\qccd@length},0);
      \draw[\qccd@zone,opacity=.55,line width=\qccd@ringwidth\QCCDUnit]
        (#1-slot-\i) circle[radius=\qccd@radius\QCCDUnit];
    }
  \end{scope}
}
\newcommand{\QCCDDrawJunction}[1]{%
  \path[fill=white,draw=\csname qccd@outline@#1\endcsname,
      line width=\qccd@nodewidth\QCCDUnit]
    ($(#1)+(-\qccd@junctionradius,-\qccd@junctionradius)$)
    rectangle ($(#1)+(\qccd@junctionradius,\qccd@junctionradius)$);
}
\newcommand{\QCCDSiteLabel}[1]{%
  \edef\qccd@x{\csname qccd@x@#1\endcsname}%
  \edef\qccd@y{\csname qccd@y@#1\endcsname}%
  \edef\qccd@angle{\csname qccd@axis@#1\endcsname}%
  \ifnum\qccd@angle=90
    \pgfmathsetmacro\qccd@tx{\qccd@x+.40*\qccd@g+.2*\qccd@font}%
    \QCCDLabel[west]{\qccd@tx}{\qccd@y}{qhwInk!82}{#1}%
  \else
    \pgfmathsetmacro\qccd@ty{\qccd@y+.40*\qccd@g+.6*\qccd@font}%
    \QCCDLabel{\qccd@x}{\qccd@ty}{qhwInk!82}{#1}%
  \fi
}
\newcommand{\QCCDJunctionLabel}[1]{%
  \pgfmathsetmacro\qccd@tx{\csname qccd@x@#1\endcsname+\qccd@junctionradius+.15*\qccd@font}%
  \pgfmathsetmacro\qccd@ty{\csname qccd@y@#1\endcsname+\qccd@junctionradius+.55*\qccd@font}%
  \QCCDLabel[west]{\qccd@tx}{\qccd@ty}{qhwInk!82}{#1}%
}
% The ion occupies a named capacity slot, with the native white halo.
% Optional colour is useful for active gates; rest is the default studio state.
\newcommand{\QCCDIon}[4][qhwData]{%
  \edef\qccd@capacity{\csname qccd@cap@#3\endcsname}%
  \pgfmathsetmacro\qccd@length{min(\qccd@lencap*\qccd@g,(.30+.15*min(\qccd@slotcap,\qccd@capacity))*\qccd@g)}%
  \pgfmathsetmacro\qccd@radius{min(.13*\qccd@g,.44*\qccd@length/\qccd@capacity)}%
  \pgfmathsetmacro\qccd@halowidth{min(max(.7,.055*\qccd@g),.45*\qccd@radius)}%
  \coordinate (#2) at (#3-slot-#4);
  \path[fill=#1,draw=white,line width=\qccd@halowidth\QCCDUnit]
    (#2) circle[radius=\qccd@radius\QCCDUnit];
  \pgfmathsetmacro\qccd@labeloffset{\qccd@radius+.6*\qccd@font}%
  \ifqccdionlabels\begingroup
    \contourlength{\qccd@texthalo\QCCDUnit}%
    \node[inner sep=0pt,text=qhwInk,
      font=\fontencoding{T1}\fontfamily{phv}\fontseries{b}\selectfont
      \fontsize{\qccd@font\QCCDUnit}{\qccd@font\QCCDUnit}\selectfont]
      at ($(#2)+(0,-\qccd@labeloffset)$) {\contour{white}{\detokenize{#2}}};
  \endgroup\fi
}

% ---- Editable architecture declarations ----------------------------------
\expandafter\def\csname qccd@architecture@grid\endcsname{%
  \QCCDGeometry{72}{18}
  \def\qccd@bounds{(27.2,18.2) rectangle (288.355,403.019)}
  \def\qccd@sites{T0_0h,T0_1h,T0_2h,T0_0v,T0_1v,T1_0v,T1_1v}%
  \def\qccd@junctions{J0_0,J0_1,J0_2,J1_0,J1_1,J1_2}%
  \QCCDDeclareJunction{J0_0}{68}{59}{qhwCorner}
  \QCCDDeclareJunction{J0_1}{68}{203}{qhwGrid}
  \QCCDDeclareJunction{J0_2}{68}{347}{qhwCorner}
  \QCCDDeclareJunction{J1_0}{212}{59}{qhwCorner}
  \QCCDDeclareJunction{J1_1}{212}{203}{qhwGrid}
  \QCCDDeclareJunction{J1_2}{212}{347}{qhwCorner}
  \QCCDDeclareSite{T0_0h}{140}{59}{0}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{T0_1h}{140}{203}{0}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{T0_2h}{140}{347}{0}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{T0_0v}{68}{131}{90}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{T0_1v}{68}{275}{90}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{T1_0v}{212}{131}{90}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{T1_1v}{212}{275}{90}{qhwTrap}{2}{qhwTrap}
  \foreach \a/\b in {J0_0/T0_0h,T0_0h/J1_0,J0_1/T0_1h,T0_1h/J1_1,J0_2/T0_2h,T0_2h/J1_2,
    J0_0/T0_0v,T0_0v/J0_1,J0_1/T0_1v,T0_1v/J0_2,J1_0/T1_0v,T1_0v/J1_1,J1_1/T1_1v,T1_1v/J1_2}
    {\QCCDRail{\a}{\b}}
}
\expandafter\def\csname qccd@architecture@ring\endcsname{%
  \QCCDGeometry{36}{9}
  \def\qccd@bounds{(41.6,1.032) rectangle (248.252,199.879)}
  \def\qccd@sites{S0,S1,S2,S3,S4,S5,A0,A3}\def\qccd@junctions{}%
  \QCCDDeclareSite{S0}{68}{67}{90}{qhwData}{2}{qhwGold}
  \QCCDDeclareSite{S1}{140}{67}{0}{qhwData}{2}{qhwData}
  \QCCDDeclareSite{S2}{212}{67}{0}{qhwData}{2}{qhwCorner}
  \QCCDDeclareSite{S3}{212}{139}{90}{qhwData}{2}{qhwGold}
  \QCCDDeclareSite{S4}{140}{139}{0}{qhwData}{2}{qhwData}
  \QCCDDeclareSite{S5}{68}{139}{0}{qhwData}{2}{qhwCorner}
  \QCCDDeclareSite{A0}{68}{31}{90}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{A3}{212}{175}{90}{qhwTrap}{2}{qhwTrap}
  \draw[qhwLoop,opacity=.15,line width=15.84\QCCDUnit,line join=round,line cap=round]
    (S0)--(S1)--(S2)--(S3)--(S4)--(S5)--cycle;
  \node[inner sep=0pt,text=qhwLoop!55,font=\fontencoding{T1}\fontfamily{phv}\bfseries\fontsize{9.18bp}{9.18bp}\selectfont] at (140,95.35){L0};
  \foreach \a/\b in {S0/S1,S1/S2,S2/S3,S3/S4,S4/S5,S5/S0}{\QCCDRail{\a}{\b}}
  \QCCDRail[qhwCompute]{S0}{A0}\QCCDRail[qhwCompute]{S3}{A3}
}
\expandafter\def\csname qccd@architecture@chain\endcsname{%
  \QCCDGeometry{72}{9}
  \def\qccd@bounds{(25.4,22.3285) rectangle (308.6,122.0187)}
  \def\qccd@sites{C0,C1,C2,C3}\def\qccd@junctions{}%
  \QCCDDeclareSite{C0}{59}{66}{0}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{C1}{131}{66}{0}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{C2}{203}{66}{0}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{C3}{275}{66}{0}{qhwTrap}{2}{qhwTrap}
  \draw[qhwLoop,opacity=.15,line width=31.68\QCCDUnit,line cap=round](C0)--(C3);
  \node[inner sep=0pt,text=qhwLoop!55,font=\fontencoding{T1}\fontfamily{phv}\bfseries\fontsize{18.36bp}{18.36bp}\selectfont] at (167,50.7){P0};
  \foreach \a/\b in {C0/C1,C1/C2,C2/C3}{\QCCDRail{\a}{\b}}
}
% The chain device without its path label, for the broadcasting figure.
\expandafter\def\csname qccd@architecture@line4\endcsname{%
  \QCCDGeometry{72}{9}
  \def\qccd@bounds{(25.4,22.3285) rectangle (308.6,122.0187)}
  \def\qccd@sites{C0,C1,C2,C3}\def\qccd@junctions{}%
  \QCCDDeclareSite{C0}{59}{66}{0}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{C1}{131}{66}{0}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{C2}{203}{66}{0}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{C3}{275}{66}{0}{qhwTrap}{2}{qhwTrap}
  \foreach \a/\b in {C0/C1,C1/C2,C2/C3}{\QCCDRail{\a}{\b}}
}
% A small instance of the native drawing grammar for the recorded parity run.
% IDs S/G/P/J are aliases for artifact site indices 0/1/2/3, respectively.
% Coordinates are a compact T embedding; the program declares the actual paths.
\expandafter\def\csname qccd@architecture@parity\endcsname{%
  \QCCDGeometry{90}{15}
  \def\qccd@bounds{(10,-8) rectangle (290,196)}
  \def\qccd@sites{S,G,P}\def\qccd@junctions{J}%
  \QCCDDeclareSite{S}{55}{55}{0}{qhwData}{2}{qhwData}
  \QCCDDeclareSite{G}{245}{55}{0}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{P}{150}{150}{90}{qhwData}{1}{qhwData}
  \QCCDDeclareJunction{J}{150}{55}{qhwGrid}
  \foreach \a/\b in {S/J,J/G,P/J}{\QCCDRail{\a}{\b}}
}
% The capacity fixture calls J a junction, but allows resident ions there.
% It is consequently shown as a native capacity-bearing site, not the website's
% empty square crossing. The optional occupancy limit remains a model property.
\expandafter\def\csname qccd@architecture@capacity\endcsname{%
  \QCCDGeometry{90}{15}
  \def\qccd@bounds{(10,-8) rectangle (290,125)}
  \def\qccd@sites{S,J,G}\def\qccd@junctions{}%
  \@ifundefined{qccd@junctioncap}{\def\qccd@junctioncap{2}}{}
  \QCCDDeclareSite{S}{55}{55}{0}{qhwData}{1}{qhwData}
  \QCCDDeclareSite{J}{150}{55}{0}{qhwData}{\qccd@junctioncap}{qhwGold}
  \QCCDDeclareSite{G}{245}{55}{0}{qhwTrap}{2}{qhwTrap}
  \foreach \a/\b in {S/J,J/G}{\QCCDRail{\a}{\b}}
}
% The running-example device of Section 2: storage S, transit site J and
% gate zone G, joined by the declared path p0: S -> J -> G.
\expandafter\def\csname qccd@architecture@primer\endcsname{%
  \QCCDGeometry{80}{20}
  \def\qccd@bounds{(-8,-20) rectangle (238,62)}
  \def\qccd@sites{S,J,G}\def\qccd@junctions{}%
  \QCCDDeclareSite{S}{25}{25}{0}{qhwData}{1}{qhwData}
  \QCCDDeclareSite{J}{110}{25}{0}{qhwData}{1}{qhwGold}
  \QCCDDeclareSite{G}{200}{25}{0}{qhwTrap}{2}{qhwTrap}
  \foreach \a/\b in {S/J,J/G}{\QCCDRail{\a}{\b}}
}
% The device of the compilation example (Sections 4 and 5): a 2 x 3 grid of
% two-ion traps, A0..A2 above and B0..B2 below three junctions on one bus.
\expandafter\def\csname qccd@architecture@grid2x3\endcsname{%
  \QCCDGeometry{60}{15}
  \def\qccd@bounds{(0,0) rectangle (272,190)}
  \def\qccd@sites{A0,A1,A2,B0,B1,B2}\def\qccd@junctions{J0,J1,J2}%
  \QCCDDeclareSite{A0}{36}{30}{90}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{A1}{136}{30}{90}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{A2}{236}{30}{90}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{B0}{36}{160}{90}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{B1}{136}{160}{90}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareSite{B2}{236}{160}{90}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareJunction{J0}{36}{95}{qhwGrid}
  \QCCDDeclareJunction{J1}{136}{95}{qhwGrid}
  \QCCDDeclareJunction{J2}{236}{95}{qhwGrid}
  \foreach \a/\b in {A0/J0,J0/B0,A1/J1,J1/B1,A2/J2,J2/B2,J0/J1,J1/J2}{\QCCDRail{\a}{\b}}
}
% Devices of the baseline-defect figure: one three-ion trap with rail stubs,
% three such traps in a line, and one junction with four arms, two of them
% with a one-ion site.
\expandafter\def\csname qccd@architecture@bugtrap\endcsname{%
  \QCCDGeometry{80}{20}
  \def\qccd@bounds{(-56,-30) rectangle (56,30)}
  \def\qccd@sites{T}\def\qccd@junctions{}%
  \QCCDDeclareSite{T}{0}{0}{0}{qhwTrap}{3}{qhwTrap}
  \draw[qhwRail,line width=\qccd@railwidth\QCCDUnit] (-54,0)--(54,0);
}
\expandafter\def\csname qccd@architecture@bugline\endcsname{%
  \QCCDGeometry{80}{20}
  \def\qccd@bounds{(-40,-30) rectangle (360,30)}
  \def\qccd@sites{T0,T1,T2}\def\qccd@junctions{}%
  \QCCDDeclareSite{T0}{0}{0}{0}{qhwTrap}{3}{qhwTrap}
  \QCCDDeclareSite{T1}{110}{0}{0}{qhwTrap}{3}{qhwTrap}
  \QCCDDeclareSite{T2}{220}{0}{0}{qhwTrap}{3}{qhwTrap}
  \foreach \a/\b in {T0/T1,T1/T2}{\QCCDRail{\a}{\b}}
}
\expandafter\def\csname qccd@architecture@bugcross\endcsname{%
  \QCCDGeometry{56}{14}
  \def\qccd@bounds{(-80,-46) rectangle (70,32)}
  \def\qccd@sites{W,N}\def\qccd@junctions{J}%
  \QCCDDeclareJunction{J}{0}{0}{qhwCorner}
  \QCCDDeclareSite{W}{-58}{0}{0}{qhwTrap}{1}{qhwTrap}
  \QCCDDeclareSite{N}{0}{-32}{90}{qhwTrap}{1}{qhwTrap}
  \draw[qhwRail,line width=\qccd@railwidth\QCCDUnit] (W)--(62,0) (N)--(0,30);
}
% The agent-designed device of the design-search figure: one line of 19
% traps, drawn one adder block per row (C carry, S store, M meeting trap,
% A, Y and D gate traps). Gate traps are teal and storage traps grey, as in
% the running example. Use with \QCCDLongTraps.
\newcommand{\qccd@adderrow}[3]{% block, carry site, y
  \QCCDDeclareSite{#2}{18}{#3}{0}{qhwData}{1}{qhwData}
  \QCCDDeclareSite{S#1}{70}{#3}{0}{qhwData}{1}{qhwData}
  \QCCDDeclareSite{M#1}{134}{#3}{0}{qhwTrap}{3}{qhwTrap}
  \QCCDDeclareSite{A#1}{210}{#3}{0}{qhwTrap}{3}{qhwTrap}
  \QCCDDeclareSite{Y#1}{298}{#3}{0}{qhwTrap}{5}{qhwTrap}
  \QCCDDeclareSite{D#1}{380}{#3}{0}{qhwTrap}{2}{qhwTrap}
  \foreach \a/\b in {#2/S#1,S#1/M#1,M#1/A#1,A#1/Y#1,Y#1/D#1}{\QCCDRail{\a}{\b}}}
\expandafter\def\csname qccd@architecture@agentadder\endcsname{%
  \QCCDGeometry{80}{8}
  \def\qccd@bounds{(-16,-20) rectangle (484,120)}
  \def\qccd@sites{C24,S0,M0,A0,Y0,D0,C25,S1,M1,A1,Y1,D1,C26,S2,M2,A2,Y2,D2,C27}%
  \def\qccd@junctions{}%
  \qccd@adderrow{0}{C24}{0}\qccd@adderrow{1}{C25}{42}\qccd@adderrow{2}{C26}{84}
  \QCCDDeclareSite{C27}{450}{84}{0}{qhwData}{3}{qhwData}
  \QCCDRail{D2}{C27}
  % the line continues from the end of one row to the start of the next
  \foreach \y in {0,42}{\draw[qhwRail,line width=\qccd@railwidth\QCCDUnit] (380,\y)--(426,\y);}
  \foreach \y in {42,84}{\draw[qhwRail,line width=\qccd@railwidth\QCCDUnit] (-14,\y)--(18,\y);}
}
% The agent's device for 32-qubit Bernstein-Vazirani: the central qubit starts alone in
% S and visits the gate traps P, A, B, C, D, E, whose capacities 11, 11, 8, 5,
% 4, 3 shrink along its walk; X and Y are four-way junctions and R is a spare
% trap that stays empty. Use with \QCCDLongTraps.
\expandafter\def\csname qccd@architecture@agenttaper\endcsname{%
  \QCCDGeometry{36}{8}
  \def\qccd@bounds{(-4,2) rectangle (296,182)}
  \def\qccd@sites{P,S,A,B,C,D,E,R}%
  \def\qccd@junctions{X,Y}%
  \QCCDDeclareSite{P}{40}{100}{0}{qhwTrap}{11}{qhwTrap}
  \QCCDDeclareSite{S}{98}{100}{0}{qhwTrap}{2}{qhwTrap}
  \QCCDDeclareJunction{X}{130}{100}{qhwGrid}
  \QCCDDeclareJunction{Y}{196}{100}{qhwGrid}
  \QCCDDeclareSite{A}{130}{44}{90}{qhwTrap}{11}{qhwTrap}
  \QCCDDeclareSite{B}{130}{148}{90}{qhwTrap}{8}{qhwTrap}
  \QCCDDeclareSite{C}{196}{60}{90}{qhwTrap}{5}{qhwTrap}
  \QCCDDeclareSite{D}{196}{137}{90}{qhwTrap}{4}{qhwTrap}
  \QCCDDeclareSite{E}{231}{100}{0}{qhwTrap}{3}{qhwTrap}
  \QCCDDeclareSite{R}{272}{100}{0}{qhwTrap}{4}{qhwTrap}
  \draw[qhwRail,line width=\qccd@railwidth\QCCDUnit]
    (P)--(R) (A)--(B) (C)--(D);
}
% A two-row ladder of four 12-ion traps. Use with \QCCDLongTraps.
\expandafter\def\csname qccd@architecture@ladderfour\endcsname{%
  \QCCDGeometry{80}{8}
  \def\qccd@bounds{(-4,-20) rectangle (370,62)}
  \def\qccd@sites{T0,T1,T2,T3}\def\qccd@junctions{}%
  \QCCDDeclareSite{T0}{84}{0}{0}{qhwTrap}{12}{qhwTrap}
  \QCCDDeclareSite{T1}{282}{0}{0}{qhwTrap}{12}{qhwTrap}
  \QCCDDeclareSite{T2}{84}{38}{0}{qhwTrap}{12}{qhwTrap}
  \QCCDDeclareSite{T3}{282}{38}{0}{qhwTrap}{12}{qhwTrap}
  \draw[qhwRail,line width=\qccd@railwidth\QCCDUnit]
    (T0)--(T1) (T2)--(T3) (T0)--(T2) (T1)--(T3);
}
% Draw a named architecture with an explicit label size (in scene units), so
% that small renderings inside figures keep legible identifiers.
\newcommand{\QCCDDevice}[2]{%
  \csname qccd@architecture@#1\endcsname
  \def\qccd@font{#2}\pgfmathsetmacro\qccd@texthalo{.14*#2}%
  \foreach \id in \qccd@sites{\QCCDDrawSite{\id}}
  \ifx\qccd@junctions\@empty\else
    \foreach \id in \qccd@junctions{\QCCDDrawJunction{\id}}\fi
}
% A label-free thumbnail of a named architecture at the given height.
\newcommand{\QCCDThumb}[2]{\resizebox{!}{#2}{%
  \begin{tikzpicture}[x=\QCCDUnit,y=-\QCCDUnit]\qccdpadsfalse
    \QCCDDevice{#1}{1}\pgfresetboundingbox
    \path[use as bounding box] \qccd@bounds;
  \end{tikzpicture}}}
\newcommand{\QCCDHardware}[1]{%
  \csname qccd@architecture@#1\endcsname
  \foreach \id in \qccd@sites{\QCCDDrawSite{\id}}
  \ifx\qccd@junctions\@empty\else
    \foreach \id in \qccd@junctions{\QCCDDrawJunction{\id}}\fi
  \foreach \id in \qccd@sites{\expandafter\QCCDSiteLabel\expandafter{\id}}
  \ifx\qccd@junctions\@empty\else
    \foreach \id in \qccd@junctions{\expandafter\QCCDJunctionLabel\expandafter{\id}}\fi
}
% ---- Named snapshots: each placement is one readable line -----------------
\expandafter\def\csname qccd@scene@grid-initial\endcsname{\QCCDHardware{grid}
  \QCCDIon{q0}{T0_1v}{0}\QCCDIon{q1}{T0_1h}{0}
  \QCCDIon{q2}{T0_0v}{0}\QCCDIon{q3}{T0_0h}{0}}
\expandafter\def\csname qccd@scene@grid-hops\endcsname{\QCCDHardware{grid}\QCCDIon{q}{T0_1h}{0}}
\expandafter\def\csname qccd@scene@grid-meeting\endcsname{\QCCDHardware{grid}
  \QCCDIon{q0}{T0_1h}{0}\QCCDIon{q1}{T0_1h}{1}
  \QCCDIon{q2}{T0_0h}{0}\QCCDIon{q3}{T0_0h}{1}}
\expandafter\def\csname qccd@scene@ring-empty\endcsname{\QCCDHardware{ring}}
\expandafter\def\csname qccd@scene@chain-empty\endcsname{\QCCDHardware{chain}}
\expandafter\def\csname qccd@scene@ring-0\endcsname{\QCCDHardware{ring}
  \QCCDIon{q0}{A0}{0}\QCCDIon{q1}{S0}{0}\QCCDIon{q2}{S2}{0}\QCCDIon{q3}{S4}{0}}
\expandafter\def\csname qccd@scene@ring-1\endcsname{\QCCDHardware{ring}
  \QCCDIon{q0}{A0}{0}\QCCDIon{q1}{S4}{0}\QCCDIon{q2}{S0}{0}\QCCDIon{q3}{S2}{0}}
\expandafter\def\csname qccd@scene@ring-2\endcsname{\QCCDHardware{ring}
  \QCCDIon{q0}{A0}{0}\QCCDIon{q1}{S2}{0}\QCCDIon{q2}{S4}{0}\QCCDIon{q3}{S0}{0}}
% Pipeline states describe placement before/after the named move and CX.
% Ion glyphs alone do not assert a quantum state or animate an unmeasured trace.
\expandafter\def\csname qccd@scene@chain-before\endcsname{\QCCDHardware{chain}
  \QCCDIon{q0}{C1}{0}\QCCDIon{q1}{C0}{0}}
\expandafter\def\csname qccd@scene@chain-after\endcsname{\QCCDHardware{chain}
  \QCCDIon{q1}{C0}{0}\QCCDIon{q0}{C0}{1}}
\expandafter\def\csname qccd@scene@ring-before\endcsname{\QCCDHardware{ring}
  \QCCDIon{q0}{A0}{0}\QCCDIon{q1}{S0}{0}}
\expandafter\def\csname qccd@scene@ring-after\endcsname{\QCCDHardware{ring}
  \QCCDIon{q0}{A0}{0}\QCCDIon{q1}{A0}{1}}
% Recorded parity states: steps 3, 5 and 6 are the three transport cycles.
\expandafter\def\csname qccd@scene@parity-empty\endcsname{\QCCDHardware{parity}}
\expandafter\def\csname qccd@scene@parity-initial\endcsname{\QCCDHardware{parity}
  \QCCDIon{q0}{S}{0}\QCCDIon{q1}{S}{1}\QCCDIon{q2}{G}{0}}
\expandafter\def\csname qccd@scene@parity-q0-in\endcsname{\QCCDHardware{parity}
  \QCCDIon{q1}{S}{0}\QCCDIon{q2}{G}{0}\QCCDIon{q0}{G}{1}}
\expandafter\def\csname qccd@scene@parity-q0-return\endcsname{\QCCDHardware{parity}
  \QCCDIon{q0}{S}{0}\QCCDIon{q1}{S}{1}\QCCDIon{q2}{G}{0}}
\expandafter\def\csname qccd@scene@parity-q1-in\endcsname{\QCCDHardware{parity}
  \QCCDIon{q0}{S}{0}\QCCDIon{q2}{G}{0}\QCCDIon{q1}{G}{1}}
\newcommand{\QCCDParityArrow}[1]{%
  \ifnum#1=0
    \draw[-{Stealth[length=3.75bp,width=3bp]},qblue,line width=1.2\QCCDUnit]
      (55,9)--(245,9);
  \else
    \draw[-{Stealth[length=3.75bp,width=3bp]},qblue,line width=1.2\QCCDUnit]
      (245,9)--(55,9);
  \fi}
\expandafter\def\csname qccd@scene@parity-q0-route\endcsname{%
  \csname qccd@scene@parity-initial\endcsname\QCCDParityArrow{0}}
\expandafter\def\csname qccd@scene@parity-q0-return-route\endcsname{%
  \csname qccd@scene@parity-q0-in\endcsname\QCCDParityArrow{1}}
\expandafter\def\csname qccd@scene@parity-q1-route\endcsname{%
  \csname qccd@scene@parity-q0-return\endcsname\QCCDParityArrow{0}}
\expandafter\def\csname qccd@scene@capacity-before\endcsname{\QCCDHardware{capacity}
  \QCCDIon{q0}{S}{0}\QCCDIon{q1}{J}{0}}
\expandafter\def\csname qccd@scene@capacity-middle\endcsname{\QCCDHardware{capacity}
  \QCCDIon{q0}{S}{0}\QCCDIon{q1}{G}{0}}
\expandafter\def\csname qccd@scene@capacity-after\endcsname{\QCCDHardware{capacity}
  \QCCDIon{q1}{G}{0}\QCCDIon{q0}{G}{1}}
\expandafter\def\csname qccd@scene@capacity-one-before\endcsname{%
  \def\qccd@junctioncap{1}\csname qccd@scene@capacity-before\endcsname}
\expandafter\def\csname qccd@scene@capacity-one-middle\endcsname{%
  \def\qccd@junctioncap{1}\csname qccd@scene@capacity-middle\endcsname}
\expandafter\def\csname qccd@scene@capacity-one-after\endcsname{%
  \def\qccd@junctioncap{1}\csname qccd@scene@capacity-after\endcsname}
\expandafter\def\csname qccd@scene@grid-route\endcsname{%
  \csname qccd@scene@grid-initial\endcsname
  \draw[-{Stealth[length=5.25bp,width=3.75bp]},qblue,line width=1.6\QCCDUnit]
    (68,251)--(68,203)--(107,203);}
\expandafter\def\csname qccd@scene@ring-route\endcsname{%
  \csname qccd@scene@ring-before\endcsname
  \draw[-{Stealth[length=3bp,width=2.25bp]},qblue,line width=.9\QCCDUnit]
    (44,67)--(44,31);}
\expandafter\def\csname qccd@scene@chain-route\endcsname{%
  \csname qccd@scene@chain-before\endcsname
  \draw[-{Stealth[length=4.5bp,width=3bp]},qblue,line width=1.4\QCCDUnit]
    (131,29)--(59,29);}
\expandafter\def\csname qccd@scene@chain-capacity\endcsname{%
  \QCCDHardware{chain}
  \QCCDIon{q1}{C0}{0}\QCCDIon{q0}{C1}{0}\QCCDIon{q2}{C2}{0}
  \draw[-{Stealth[length=4.5bp,width=3bp]},qblue,line width=1.4\QCCDUnit]
    (131,29)--(59,29);}
\newcommand{\QCCDScene}[2][]{%
  \begin{tikzpicture}[x=\QCCDUnit,y=-\QCCDUnit,transform shape,#1]
    \csname qccd@scene@#2\endcsname
    \pgfresetboundingbox
    \path[use as bounding box] \qccd@bounds;
  \end{tikzpicture}%
}
\makeatother

